Effective and Efficient Computation with Multiple-timescale Spiking Recurrent Neural Networks

The emergence of brain-inspired neuromorphic computing as a paradigm for edge AI is motivating the search for high-performance and efficient spiking neural networks to run on this hardware. However, compared to classical neural networks in deep learning, current spiking neural networks lack competitive performance in compelling areas. Here, for sequential and streaming tasks, we demonstrate how a novel type of adaptive spiking recurrent neural network (SRNN) is able to achieve state-of-the-art performance compared to other spiking neural networks and almost reach or exceed the performance of classical recurrent neural networks (RNNs) while exhibiting sparse activity. From this, we calculate a $>$100x energy improvement for our SRNNs over classical RNNs on the harder tasks. To achieve this, we model standard and adaptive multiple-timescale spiking neurons as self-recurrent neural units, and leverage surrogate gradients and auto-differentiation in the PyTorch Deep Learning framework to efficiently implement backpropagation-through-time, including learning of the important spiking neuron parameters to adapt our spiking neurons to the tasks.

==> 1_Abstract.tex <==
% \begin{abstract}

% \begin{itemize}
% 	\item SNNs binary neurons with (self-)memory. 
% 	\item Lack of exciting applications compared to DNNs due to combination of (lack of) suitable benchmarks and lack of effective algorithms due to discontinuity of spiking process. Recent work has suggested how to overcome this. 
% 	\item Here, study streaming tasks with low-dimensional inputs. Streaming: continuous input, limited latency (buffering). Low-dimensional due to capacity of software frameworks (essentially RNNs), applications for ultra-low power IoT hardware.  
% 	\item main contribution: allow neural parameters to be learned alongside weights, this makes a massive difference in performance, achieve 100x increase in efficiency compared to equivalent ANN.
% 	\item secondary contribution: we use a multi-gaussian surrogate gradient, which improves performance and sparsity of the network activity. [CHECK IN DATA]
% 	\item secondary contribution: demonstrate that more complex SNN models with multiple adaptable time-scales strongly increase SNN performance. 
% 	\item secondary contribution: report on activations/energy use ... (TODO)
% 	\item secondary contribution: we find that self-recurrent connections as in SNNs are powerful, non-spiking versions of the network slighlty outperform spiking versions. 
% 	\item Tasks: ECG, S-MNIST, PS-MNIST, SHD.
% 	\item Achieve SoTa for SNNs, exceed standard DNNs for ECG, PS-MNIST, S-MNIST, approach SoTa DNNs for S-MNIST
% \end{itemize}

% % 1. (use case)Spiking neural networks (SNNs) are believed to be the next generation neural network with computationally and energy-efficient for real-time solutions. But there isn't any good use case found for SNN to show its advantages. 

% % 2. (gradient)In another view, many researchers are working to find an efficient learning algorithm within both supervised and unsupervised framework. Due to the non-differential propriety in SNN, all methods need to generate or calculate the "gradients" for weight updating. (some paper generate the gradients from the neuron activities). With surrogate gradient, We've got near sota performance in some typical classification dataset.
% % 3. possibility on hardware. FPGA implementation, always-on device, low energy cost.
% % 4. The streaming task, as well as the Many-to-Many task, which refers to the situation where the many inputs are read to give the same number of output. In steaming task, we prefer to receive the result from the model when the input is given.
% % In this paper, we find out the SNNs performs better than LSTMs, GRUs in terms of both accuracy and energy efficiency with the help of the adaptive neuron's internal dynamic modelling capability on ECG streaming task.


% % 2) computation is event-driven and there is no clock or fixed time at which the computation happen, only when data is transmitted, ECG is sparse. so many zeros.
% % 3) the architecture of the network is truly scalable and works in parallel (non-Von Neumann!)
% % 4) by having a recurrent neural network we exploit the same computational unit over time, this means that we can have complex spatio-temporal dynamics with very little neurons, but highly interconnected. In this way we can solve complex spatio-temporal tasks.

% \end{abstract}

==> references.tex <==

%state of the art SNN
@article{sengupta2019going,
  title={Going deeper in spiking neural networks: Vgg and residual architectures},
  author={Sengupta, Abhronil and Ye, Yuting and Wang, Robert and Liu, Chiao and Roy, Kaushik},
  journal={Frontiers in neuroscience},
  volume={13},
  year={2019},
  publisher={Frontiers Media SA}
}

@article{hurst1998naming,
  title={Naming of the waves in the ECG, with a brief account of their genesis},
  author={Hurst, J Willis},
  journal={Circulation},
  volume={98},
  number={18},
  pages={1937--1942},
  year={1998},
  publisher={Am Heart Assoc}
}

@inproceedings{huh2018gradient,
  title={Gradient descent for spiking neural networks},
  author={Huh, Dongsung and Sejnowski, Terrence J},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1433--1443},
  year={2018}
}

@article{attwell2001energy,
  title={An energy budget for signaling in the grey matter of the brain},
  author={Attwell, David and Laughlin, Simon B},
  journal={Journal of Cerebral Blood Flow \& Metabolism},
  volume={21},
  number={10},
  pages={1133--1145},
  year={2001},
  publisher={SAGE Publications Sage UK: London, England}
}

@book{maass2001pulsed,
  title={Pulsed neural networks},
  author={Maass, Wolfgang and Bishop, Christopher M},
  year={2001},
  publisher={MIT press}
}

@article{wang2020-uq,
  title={Temporal Pulses Driven Spiking Neural Network for Fast Object Recognition in Autonomous Driving},
  author={Wang, Wei and Zhou, Shibo and Li, Jingxi and Li, Xiaohua and Yuan, Junsong and Jin, Zhanpeng},
  journal={arXiv preprint arXiv:2001.09220},
  year={2020}
}

@article{benidis2020neural,
  title={Neural forecasting: Introduction and literature overview},
  author={Benidis, Konstantinos and Rangapuram, Syama Sundar and Flunkert, Valentin and Wang, Bernie and Maddix, Danielle and Turkmen, Caner and Gasthaus, Jan and Bohlke-Schneider, Michael and Salinas, David and Stella, Lorenzo and others},
  journal={arXiv preprint arXiv:2004.10240},
  year={2020}
}

@article{oord2016wavenet,
  title={Wavenet: A generative model for raw audio},
  author={Oord, Aaron van den and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray},
  journal={arXiv preprint arXiv:1609.03499},
  year={2016}
}

@ARTICLE{OConnor2013-un,
  title     = "Real-time classification and sensor fusion with a spiking deep
               belief network",
  author    = "O'Connor, Peter and Neil, Daniel and Liu, Shih-Chii and
               Delbruck, Tobi and Pfeiffer, Michael",
  abstract  = "Deep Belief Networks (DBNs) have recently shown impressive
               performance on a broad range of classification problems. Their
               generative properties allow better understanding of the
               performance, and provide a simpler solution for sensor fusion
               tasks. However, because of their inherent need for feedback and
               parallel update of large numbers of units, DBNs are expensive to
               implement on serial computers. This paper proposes a method
               based on the Siegert approximation for Integrate-and-Fire
               neurons to map an offline-trained DBN onto an efficient
               event-driven spiking neural network suitable for hardware
               implementation. The method is demonstrated in simulation and by
               a real-time implementation of a 3-layer network with 2694
               neurons used for visual classification of MNIST handwritten
               digits with input from a 128 $\times$ 128 Dynamic Vision Sensor
               (DVS) silicon retina, and sensory-fusion using additional input
               from a 64-channel AER-EAR silicon cochlea. The system is
               implemented through the open-source software in the jAER project
               and runs in real-time on a laptop computer. It is demonstrated
               that the system can recognize digits in the presence of
               distractions, noise, scaling, translation and rotation, and that
               the degradation of recognition performance by using an
               event-based approach is less than 1\%. Recognition is achieved
               in an average of 5.8 ms after the onset of the presentation of a
               digit. By cue integration from both silicon retina and cochlea
               outputs we show that the system can be biased to select the
               correct digit from otherwise ambiguous input.",
  journal   = "Front. Neurosci.",
  publisher = "frontiersin.org",
  volume    =  7,
  pages     = "178",
  month     =  oct,
  year      =  2013,
  keywords  = "deep belief networks; deep learning; generative model; sensory
               fusion; silicon cochlea; silicon retina; spiking neural network",
  language  = "en"
}


@BOOK{Gerstner2002-wd,
  title     = "Spiking Neuron Models: Single Neurons, Populations, Plasticity",
  author    = "Gerstner, Wulfram and Kistler, Werner M",
  abstract  = "Neurons in the brain communicate by short electrical pulses, the
               so-called action potentials or spikes. How can we understand the
               process of spike generation? How can we understand information
               transmission by neurons? What happens if thousands of neurons
               are coupled together in a seemingly random network? How does the
               network connectivity determine the activity patterns? And, vice
               versa, how does the spike activity influence the connectivity
               pattern? These questions are addressed in this 2002 introduction
               to spiking neurons aimed at those taking courses in
               computational neuroscience, theoretical biology, biophysics, or
               neural networks. The approach will suit students of physics,
               mathematics, or computer science; it will also be useful for
               biologists who are interested in mathematical modelling. The
               text is enhanced by many worked examples and illustrations.
               There are no mathematical prerequisites beyond what the audience
               would meet as undergraduates: more advanced techniques are
               introduced in an elementary, concrete fashion when needed.",
  publisher = "Cambridge University Press",
  month     =  aug,
  year      =  2002,
  language  = "en"
}


@ARTICLE{Roy2019-rv,
  title    = "Towards spike-based machine intelligence with neuromorphic
              computing",
  author   = "Roy, Kaushik and Jaiswal, Akhilesh and Panda, Priyadarshini",
  abstract = "Guided by brain-like 'spiking' computational frameworks,
              neuromorphic computing-brain-inspired computing for machine
              intelligence-promises to realize artificial intelligence while
              reducing the energy requirements of computing platforms. This
              interdisciplinary field began with the implementation of silicon
              circuits for biological neural routines, but has evolved to
              encompass the hardware implementation of algorithms with
              spike-based encoding and event-driven representations. Here we
              provide an overview of the developments in neuromorphic computing
              for both algorithms and hardware and highlight the fundamentals
              of learning and hardware frameworks. We discuss the main
              challenges and the future prospects of neuromorphic computing,
              with emphasis on algorithm-hardware codesign.",
  journal  = "Nature",
  volume   =  575,
  number   =  7784,
  pages    = "607--617",
  month    =  nov,
  year     =  2019,
  language = "en"
}


@article{xu2015empirical,
  title={Empirical evaluation of rectified activations in convolutional network},
  author={Xu, Bing and Wang, Naiyan and Chen, Tianqi and Li, Mu},
  journal={arXiv preprint arXiv:1505.00853},
  year={2015}
}

@article{izhikevich2003simple,
  title={Simple model of spiking neurons},
  author={Izhikevich, Eugene M},
  journal={IEEE Transactions on neural networks},
  volume={14},
  number={6},
  pages={1569--1572},
  year={2003},
  publisher={IEEE}
}

@article{le2015simple,
  title={A simple way to initialize recurrent networks of rectified linear units},
  author={Le, Quoc V and Jaitly, Navdeep and Hinton, Geoffrey E},
  journal={arXiv preprint arXiv:1504.00941},
  year={2015}
}

% efficientNET
@article{tan2019efficientnet,
  title={Efficientnet: Rethinking model scaling for convolutional neural networks},
  author={Tan, Mingxing and Le, Quoc V},
  journal={arXiv preprint arXiv:1905.11946},
  year={2019}
}

% energy-efficient designing
@inproceedings{yang2017designing,
  title={Designing energy-efficient convolutional neural networks using energy-aware pruning},
  author={Yang, Tien-Ju and Chen, Yu-Hsin and Sze, Vivienne},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5687--5695},
  year={2017}
}

% network in network nin
@article{lin2013network,
  title={Network in network},
  author={Lin, Min and Chen, Qiang and Yan, Shuicheng},
  journal={arXiv preprint arXiv:1312.4400},
  year={2013}
}

@article{iandola2016squeezenet,
  title={SqueezeNet: AlexNet-level accuracy with 50x fewer parameters and< 0.5 MB model size},
  author={Iandola, Forrest N and Han, Song and Moskewicz, Matthew W and Ashraf, Khalid and Dally, William J and Keutzer, Kurt},
  journal={arXiv preprint arXiv:1602.07360},
  year={2016}
}
% resnet
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}
% binaryconnect
@inproceedings{courbariaux2015binaryconnect,
  title={Binaryconnect: Training deep neural networks with binary weights during propagations},
  author={Courbariaux, Matthieu and Bengio, Yoshua and David, Jean-Pierre},
  booktitle={Advances in neural information processing systems},
  pages={3123--3131},
  year={2015}
}

% DSQ
@inproceedings{gong2019differentiable,
  title={Differentiable soft quantization: Bridging full-precision and low-bit neural networks},
  author={Gong, Ruihao and Liu, Xianglong and Jiang, Shenghu and Li, Tianxiang and Hu, Peng and Lin, Jiazhen and Yu, Fengwei and Yan, Junjie},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={4852--4861},
  year={2019}
}

% XNOR net
@inproceedings{rastegari2016xnor,
  title={Xnor-net: Imagenet classification using binary convolutional neural networks},
  author={Rastegari, Mohammad and Ordonez, Vicente and Redmon, Joseph and Farhadi, Ali},
  booktitle={European conference on computer vision},
  pages={525--542},
  year={2016},
  organization={Springer}
}
% BNN+
@article{darabi2018bnn+,
  title={BNN+: Improved binary network training},
  author={Darabi, Sajad and Belbahri, Mouloud and Courbariaux, Matthieu and Nia, Vahid Partovi},
  journal={arXiv preprint arXiv:1812.11800},
  year={2018}
}

% DVS sensor
@article{lichtsteiner2008128,
  title={A 128x128 120 dB 15$\mu$s Latency Asynchronous Temporal Contrast Vision Sensor},
  author={Lichtsteiner, Patrick and Posch, Christoph and Delbruck, Tobi},
  journal={IEEE journal of solid-state circuits},
  volume={43},
  number={2},
  pages={566--576},
  year={2008},
  publisher={IEEE}
}

% SNN and ANN energy on image classification
@article{panda2019towards,
  title={Towards Scalable, Efficient and Accurate Deep Spiking Neural Networks with Backward Residual Connections, Stochastic Softmax and Hybridization},
  author={Panda, Priyadarshini and Aketi, Aparna and Roy, Kaushik},
  journal={arXiv preprint arXiv:1910.13931},
  year={2019}
}

% snn conversion1
@article{zambrano2016fast,
  title={Fast and efficient asynchronous neural computation with adapting spiking neural networks},
  author={Zambrano, Davide and Bohte, Sander M},
  journal={arXiv preprint arXiv:1609.02053},
  year={2016}
}
% Training Deep Spiking Neural Networks Using Backpropagation
@article{lee2016training,
  title={Training deep spiking neural networks using backpropagation},
  author={Lee, Jun Haeng and Delbruck, Tobi and Pfeiffer, Michael},
  journal={Frontiers in neuroscience},
  volume={10},
  pages={508},
  year={2016},
  publisher={Frontiers}
}

@article{maass1997networks,
  title={Networks of spiking neurons: the third generation of neural network models},
  author={Maass, Wolfgang},
  journal={Neural networks},
  volume={10},
  number={9},
  pages={1659--1671},
  year={1997},
  publisher={Elsevier}
}

% bohte BP
@inproceedings{bohte2011error,
  title={Error-backpropagation in networks of fractionally predictive spiking neurons},
  author={Bohte, Sander M},
  booktitle={International Conference on Artificial Neural Networks},
  pages={60--68},
  year={2011},
  organization={Springer}
}
% Loihi
@article{davies2018loihi,
  title={Loihi: A neuromorphic manycore processor with on-chip learning},
  author={Davies, Mike and Srinivasa, Narayan and Lin, Tsung-Han and Chinya, Gautham and Cao, Yongqiang and Choday, Sri Harsha and Dimou, Georgios and Joshi, Prasad and Imam, Nabil and Jain, Shweta and others},
  journal={IEEE Micro},
  volume={38},
  number={1},
  pages={82--99},
  year={2018},
  publisher={IEEE}
}

% mixed learning
@inproceedings{zhang2018plasticity,
  title={A plasticity-centric approach to train the non-differential spiking neural networks},
  author={Zhang, Tielin and Zeng, Yi and Zhao, Dongcheng and Shi, Mengting},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}
% cnn ECG
@article{rajpurkar2017cardiologist,
  title={Cardiologist-level arrhythmia detection with convolutional neural networks},
  author={Rajpurkar, Pranav and Hannun, Awni Y and Haghpanahi, Masoumeh and Bourn, Codie and Ng, Andrew Y},
  journal={arXiv preprint arXiv:1707.01836},
  year={2017}
}

% LSTM
@article{gers1999learning,
  title={Learning to forget: Continual prediction with LSTM},
  author={Gers, Felix A and Schmidhuber, J{\"u}rgen and Cummins, Fred},
  year={1999},
  publisher={IET}
}
% GRU
@article{chung2014empirical,
  title={Empirical evaluation of gated recurrent neural networks on sequence modeling},
  author={Chung, Junyoung and Gulcehre, Caglar and Cho, KyungHyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1412.3555},
  year={2014}
}
% BPTT
@article{werbos1990backpropagation,
  title={Backpropagation through time: what it does and how to do it},
  author={Werbos, Paul J},
  journal={Proceedings of the IEEE},
  volume={78},
  number={10},
  pages={1550--1560},
  year={1990},
  publisher={IEEE}
}

% wavelet Bir-LSTM ECG
@article{yildirim2018novel,
  title={A novel wavelet sequence based on deep bidirectional LSTM network model for ECG signal classification},
  author={Yildirim, {\"O}zal},
  journal={Computers in biology and medicine},
  volume={96},
  pages={189--202},
  year={2018},
  publisher={Elsevier}
}

% MIT-BIH
@article{alfaras2019fast,
  title={A fast machine learning model for ECG-based heartbeat classification and arrhythmia detection},
  author={Alfaras, Miquel and Soriano, Miguel Cornelles and Ort{\'\i}n, Silvia},
  journal={Frontiers in Physics},
  volume={7},
  pages={103},
  year={2019},
  publisher={Frontiers}
}
% MIT-BIH
@inproceedings{kachuee2018ecg,
  title={Ecg heartbeat classification: A deep transferable representation},
  author={Kachuee, Mohammad and Fazeli, Shayan and Sarrafzadeh, Majid},
  booktitle={2018 IEEE International Conference on Healthcare Informatics (ICHI)},
  pages={443--444},
  year={2018},
  organization={IEEE}
}


% Spike NN opp and challenge
@article{pfeiffer2018deep,
  title={Deep learning with spiking neurons: opportunities and challenges},
  author={Pfeiffer, Michael and Pfeil, Thomas},
  journal={Frontiers in neuroscience},
  volume={12},
  year={2018},
  publisher={Frontiers Media SA}
}
% summary on neuromorphic computing
@article{roy2019towards,
  title={Towards spike-based machine intelligence with neuromorphic computing},
  author={Roy, Kaushik and Jaiswal, Akhilesh and Panda, Priyadarshini},
  journal={Nature},
  volume={575},
  number={7784},
  pages={607--617},
  year={2019},
  publisher={Nature Publishing Group}
}

% surrogate gradeint
@article{neftci2019surrogate,
  title={Surrogate gradient learning in spiking neural networks},
  author={Neftci, Emre O and Mostafa, Hesham and Zenke, Friedemann},
  journal={arXiv preprint arXiv:1901.09948},
  year={2019}
}

% L2L spike  recurrent network
@inproceedings{bellec2018long,
  title={Long short-term memory and learning-to-learn in networks of spiking neurons},
  author={Bellec, Guillaume and Salaj, Darjan and Subramoney, Anand and Legenstein, Robert and Maass, Wolfgang},
  booktitle={Advances in Neural Information Processing Systems},
  pages={787--797},
  year={2018}
}

% SRNN 
@article{demin2018recurrent,
  title={Recurrent Spiking Neural Network Learning Based on a Competitive Maximization of Neuronal Activity},
  author={Demin, Vyacheslav and Nekhaev, Dmitry},
  journal={Frontiers in neuroinformatics},
  volume={12},
  year={2018},
  publisher={Frontiers Media SA}
}

% deep learning in srnn, section 3D is Recurrent SNNs
@article{tavanaei2019deep,
  title={Deep learning in spiking neural networks},
  author={Tavanaei, Amirhossein and Ghodrati, Masoud and Kheradpisheh, Saeed Reza and Masquelier, Timothee and Maida, Anthony},
  journal={Neural Networks},
  volume={111},
  pages={47--63},
  year={2019},
  publisher={Elsevier}
}

% weight quan]


% Blended coarse gradient descent
@article{yin2019blended,
  title={Blended coarse gradient descent for full quantization of deep neural networks},
  author={Yin, Penghang and Zhang, Shuai and Lyu, Jiancheng and Osher, Stanley and Qi, Yingyong and Xin, Jack},
  journal={Research in the Mathematical Sciences},
  volume={6},
  number={1},
  pages={14},
  year={2019},
  publisher={Springer}
}


% melodies steraming 
@article{colombo2016algorithmic,
  title={Algorithmic composition of melodies with deep recurrent neural networks},
  author={Colombo, Florian and Muscinelli, Samuel P and Seeholzer, Alexander and Brea, Johanni and Gerstner, Wulfram},
  journal={arXiv preprint arXiv:1606.07251},
  year={2016}
}

% Heidelberg dataset
@article{cramer2019heidelberg,
  title={The Heidelberg spiking datasets for the systematic evaluation of spiking neural networks},
  author={Cramer, Benjamin and Stradmann, Yannik and Schemmel, Johannes and Zenke, Friedemann},
  journal={arXiv preprint arXiv:1910.07407},
  year={2019}
}

% unsupervised MNIST 2015
@article{diehl2015unsupervised,
  title={Unsupervised learning of digit recognition using spike-timing-dependent plasticity},
  author={Diehl, Peter U and Cook, Matthew},
  journal={Frontiers in computational neuroscience},
  volume={9},
  pages={99},
  year={2015},
  publisher={Frontiers}
}

% RBF encoding
@article{bohte2002unsupervised,
  title={Unsupervised clustering with spiking neurons by sparse temporal coding and multilayer RBF networks},
  author={Bohte, Sander M and La Poutr{\'e}, Han and Kok, Joost N},
  journal={IEEE Transactions on neural networks},
  volume={13},
  number={2},
  pages={426--435},
  year={2002},
  publisher={IEEE}
}

% N_MNIST
@article{orchard2015converting,
  title={Converting static image datasets to spiking neuromorphic datasets using saccades},
  author={Orchard, Garrick and Jayawant, Ajinkya and Cohen, Gregory K and Thakor, Nitish},
  journal={Frontiers in neuroscience},
  volume={9},
  pages={437},
  year={2015},
  publisher={Frontiers}
}


% DVS RIN-DT
@article{hu2018overcoming,
  title={Overcoming the vanishing gradient problem in plain recurrent networks},
  author={Hu, Yuhuang and Huber, Adrian and Anumula, Jithendar and Liu, Shih-Chii},
  journal={arXiv preprint arXiv:1801.06105},
  year={2018}
}
@inproceedings{lichtsteiner2006128,
  title={A 128 x 128 120db 30mw asynchronous vision sensor that responds to relative intensity change},
  author={Lichtsteiner, Patrick and Posch, Christoph and Delbruck, Tobi},
  booktitle={2006 IEEE International Solid State Circuits Conference-Digest of Technical Papers},
  pages={2060--2069},
  year={2006},
  organization={IEEE}
}

% DAS
@article{liu2013asynchronous,
  title={Asynchronous Binaural Spatial Audition Sensor With 2X64X4 Channel Output},
  author={Liu, Shih-Chii and van Schaik, Andr{\'e} and Minch, Bradley A and Delbruck, Tobi},
  journal={IEEE transactions on biomedical circuits and systems},
  volume={8},
  number={4},
  pages={453--464},
  year={2013},
  publisher={IEEE}
}

% N-Digits
@article{anumula2018feature,
  title={Feature representations for neuromorphic audio spike streams},
  author={Anumula, Jithendar and Neil, Daniel and Delbruck, Tobi and Liu, Shih-Chii},
  journal={Frontiers in neuroscience},
  volume={12},
  pages={23},
  year={2018},
  publisher={Frontiers}
}

%% LSTM
@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

%% LSTM 2
@article{graves2013generating,
  title={Generating sequences with recurrent neural networks},
  author={Graves, Alex},
  journal={arXiv preprint arXiv:1308.0850},
  year={2013}
}

%% Ind RNN

@article{li2019deep,
  title={Deep Independently Recurrent Neural Network (IndRNN)},
  author={Li, Shuai and Li, Wanqing and Cook, Chris and Gao, Yanbo and Zhu, Ce},
  journal={arXiv preprint arXiv:1910.06251},
  year={2019}
}

% LSTM MNIST
@inproceedings{arjovsky2016unitary,
  title={Unitary evolution recurrent neural networks},
  author={Arjovsky, Martin and Shah, Amar and Bengio, Yoshua},
  booktitle={International Conference on Machine Learning},
  pages={1120--1128},
  year={2016}
}

% LMU
@inproceedings{voelker2019legendre,
  title={Legendre Memory Units: Continuous-Time Representation in Recurrent Neural Networks},
  author={Voelker, Aaron and Kaji{\'c}, Ivana and Eliasmith, Chris},
  booktitle={Advances in Neural Information Processing Systems},
  pages={15544--15553},
  year={2019}
}


% SLayer
@InCollection{Shrestha2018,
  author    = {Shrestha, Sumit Bam and Orchard, Garrick},
  title     = {{SLAYER}: Spike Layer Error Reassignment in Time},
  booktitle = {Advances in Neural Information Processing Systems 31},
  publisher = {Curran Associates, Inc.},
  year      = {2018},
  editor    = {S. Bengio and H. Wallach and H. Larochelle and K. Grauman and N. Cesa-Bianchi and R. Garnett},
  pages     = {1419--1428},
  url       = {http://papers.nips.cc/paper/7415-slayer-spike-layer-error-reassignment-in-time.pdf},
}
% ReSuMe
@article{ponulak2008analysis,
  title={Analysis of the ReSuMe learning process for spiking neural networks},
  author={Ponulak, Filip},
  journal={International Journal of Applied Mathematics and Computer Science},
  volume={18},
  number={2},
  pages={117--127},
  year={2008},
  publisher={Sciendo}
}

% zenkeSuperspike
@article{zenke2018superspike,
  title={Superspike: Supervised learning in multilayer spiking neural networks},
  author={Zenke, Friedemann and Ganguli, Surya},
  journal={Neural computation},
  volume={30},
  number={6},
  pages={1514--1541},
  year={2018},
  publisher={MIT Press}
}
% sander spikeprop
@inproceedings{bohte2000spikeprop,
  title={SpikeProp: backpropagation for networks of spiking neurons.},
  author={Bohte, Sander M and Kok, Joost N and La Poutr{\'e}, Johannes A},
  booktitle={ESANN},
  volume={48},
  pages={17--37},
  year={2000}
}

% mozer BPTT
@article{mozer1995focused,
  title={A focused backpropagation algorithm for temporal},
  author={Mozer, Michael C},
  journal={Backpropagation: Theory, architectures, and applications},
  volume={137},
  year={1995}
}

% ruckauer2018
@article{ruckauer2019closing,
  title={Closing the Accuracy Gap in an Event-Based Visual Recognition Task},
  author={R{\"u}ckauer, Bodo and K{\"a}nzig, Nicolas and Liu, Shih-Chii and Delbruck, Tobi and Sandamirskaya, Yulia},
  journal={arXiv preprint arXiv:1906.08859},
  year={2019}
}

%adam
@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

% spike time BP
@article{zhang2020spike,
  title={Spike-Timing-Dependent Back Propagation in Deep Spiking Neural Networks},
  author={Zhang, Malu and Wang, Jiadong and Zhang, Zhixuan and Belatreche, Ammar and Wu, Jibin and Chua, Yansong and Qu, Hong and Li, Haizhou},
  journal={arXiv preprint arXiv:2003.11837},
  year={2020}
}

% CMOS energy
@inproceedings{han2015learning,
  title={Learning both weights and connections for efficient neural network},
  author={Han, Song and Pool, Jeff and Tran, John and Dally, William},
  booktitle={Advances in neural information processing systems},
  pages={1135--1143},
  year={2015}
}


